Categorical Data Structures for Technical Computing

Many mathematical objects can be represented as functors from finitely-presented categories $\mathsf{C}$ to $\mathsf{Set}$. For instance, graphs are functors to $\mathsf{Set}$ from the category with two parallel arrows. Such functors are known informally as $\mathsf{C}$-sets. In this paper, we describe and implement an extension of $\mathsf{C}$-sets having data attributes with fixed types, such as graphs with labeled vertices or real-valued edge weights. We call such structures "acsets," short for "attributed $\mathsf{C}$-sets." Derived from previous work on algebraic databases, acsets are a joint generalization of graphs and data frames. They also encompass more elaborate graph-like objects such as wiring diagrams and Petri nets with rate constants. We develop the mathematical theory of acsets and then describe a generic implementation in the Julia programming language, which uses advanced language features to achieve performance comparable with specialized data structures.

==> figures/benchmarks.tex <==
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{figures/bm/Graph}
  \caption{Graph operations}
  \label{subfig:graph_bm}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{figures/bm/SymmetricGraph}
  \caption{Symmetric graph operations}
  \label{subfig:symmetric_graph_bm}
\end{subfigure}
\vspace{1em}
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{figures/bm/GraphConnComponents}
  \caption{Connected componenents}
  \label{subfig:graph_conn_components_bm}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{figures/bm/SymmetricGraphConnComponent}
  \caption{Connected components of symmetric graphs}
  \label{subfig:symmetric_graph_conn_components_bm}
\end{subfigure}
\vspace{1em}
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{figures/bm/WeightedGraph}
  \caption{Weighted graphs (edge attributes)}
  \label{subfig:weighted_graph_bm}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{figures/bm/LabeledGraph}
  \caption{Labeled graphs (vertex attributes)}
  \label{subfig:labeled_graph_bm}
\end{subfigure}
\vspace{1em}
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{figures/bm/RandomGraph}
  \caption{Constructing random graphs}
  \label{subfig:random_graph_bm}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{figures/bm/Searching}
  \caption{Searching in random graphs}
  \label{subfig:searching_bm}
\end{subfigure}

